A Viral Marketing-Based Model For Opinion Dynamics in Online Social Networks

Online social networks provide a medium for citizens to form opinions on different societal issues, and a forum for public discussion. They also expose users to viral content, such as breaking news articles. In this paper, we study the interplay between these two aspects: opinion formation and information cascades in online social networks. We present a new model that allows us to quantify how users change their opinion as they are exposed to viral content. Our model is a combination of the popular Friedkin--Johnsen model for opinion dynamics and the independent cascade model for information propagation. We present algorithms for simulating our model, and we provide approximation algorithms for optimizing certain network indices, such as the sum of user opinions or the disagreement--controversy index; our approach can be used to obtain insights into how much viral content can increase these indices in online social networks. Finally, we evaluate our model on real-world datasets. We show experimentally that marketing campaigns and polarizing contents have vastly different effects on the network: while the former have only limited effect on the polarization in the network, the latter can increase the polarization up to 59% even when only 0.5% of the users start sharing a polarizing content. We believe that this finding sheds some light into the growing segregation in today's online media.

==> arXiv version/online-only.tex <==
\section{Overview of the Appendix}
The appendix is organized as follows:
\begin{itemize}
	\item Sec.~\ref{sec:omitted} contains omitted proofs from the main text.
	\item Sec.~\ref{sec:comparison} presents a comparison of the
		spread--acknowledge model and the FJ model for the sum index.
	\item Sec.~\ref{sec:add-experiments} presents further experimental
		evaluation of our model and our algorithms.
\end{itemize}

\section{Omitted Proofs}
\label{sec:omitted}

\subsection{Proof of Lemma~\ref{lem:equivalence}}
\label{sec:proof-equivalence}
Before we present the formal proof, we first present a proof sketch.
\begin{proof}[Proof Sketch]
	We prove the first claim by induction over the number of rounds.
	In round~$0$, we assumed that both models were initialized with
	the same innate opinions $\begop$ and the same seed nodes. Thus, the
	distributions are deterministic and identical. Now consider round $t>0$.
	For the \spread we note that Phase~I does not change the innate opinions
	and it has no impact on Phase~II.  Therefore, we can
	ignore Phase~I and the model coincides with the two-stage model.
	Now the claim follows from the induction hypothesis.
	
	The second claim essentially follows from the fact that the expressed
	equilibrium opinions $\z^*$ and $\zz^*$ are deterministic
	transformations of $\s$ and $\ss$. 
	However, there is a	subtlety:   
	While in the two-stage model, all opinion updates (as per Equation~\eqref{eq:opinion-round}) are performed
	based on the final vector of innate opinions $\ss$, this is not the
	case in the \spread. In the \spread, it is possible that the innate
	opinions change from round to round and, therefore, it could be possible
	that the opinion updates from early rounds might alter $\z^*$ (as
	per Equation~\eqref{eq:opinion-equilibrium}).  However, we show that this is
	not the case since the equilibrium opinions $\z^*$  are independent from how
	the initial expressed opinions $z^{(0)}$ were initialized in
	Equation~\eqref{eq:opinion-round}. Thus, we can ignore all
	opinion updates that were performed while the innate opinion
	vector did not correspond to $\s$. Now, since $\s$ and $\ss$ follow
	the same distribution and since $\z^*$ and $\zz^*$ are deterministic
	transformations of $\s$ and $\ss$, we obtain the claim.
\end{proof}

Now we proceed to the formal proof of the lemma.

\begin{proof}
    First, as mentioned above, Phase~I does not change the innate opinions
	and it has no impact on Phase~II.  
     Therefore, both models must generate the same distribution over the states of the users. 
	This implies that the distribution of $\s$ and $\ss$ are the same at the end
	of the process for both models.
    The different part is, when the information spread ceases, the two-stage model 
    and \spread may have different intermediate expressed opinions. 
    Therefore, we will prove that the equilibrium expressed opinions only depend on the 
    innate opinions, rather than the intermediate expressed opinions.

   Next, we present an equivalent formulation of the update rule of the \fj.
   The new formulation allows us to give a simple proof that when the innate
   opinions change over time, then the final expressed
   opinion $\z^*$ only depends on the last vector of innate opinions; in
   particular, $\z^*$ is independent of the intermediate expressed and innate
   opinions.

   Let $\Stoc$ be an $n \times n$ row stochastic matrix, let $\Lambda$ be a $n \times n$ diagonal matrix.
   Specifically, let
   $$\eStoc{i}{j} = \frac{w_{i,j}}{\sum_{j\in N(i)}w_{i,j}}$$
   and let
   $$\Lambda_{ii} = \frac{\sum_{j\in N(i)} w_{i,j}}{1 + \sum_{j \in N(i)}
	   w_{i,j}}.$$
   The update rule of the \fj from Equation~\eqref{eq:opinion-round} can thus be 
   equivalently formulated as:
   \begin{equation}
       \label{eq:opinion-round-2}
       \finop^{(t+1)} = \Lambda \Stoc \finop^{(t)} + (\ID - \Lambda)\begop.
   \end{equation}

   The following lemma shows how the expressed opinions evolve when the vector
   of innate opinions~$\begop$ is fixed. Note that in the lemma we do not make
   the assumption that $\finop^{(t)}$ was obtained from the same vector of
   innate opinions $\begop$.
   \begin{lemma}
      \label{lemma:opinion-model-1}
       Consider the vector of innate opinions $\begop$ and the expressed opinions
	   $\finop^{(t)}$ at time step $t$. 
	   Suppose that we perform $T$ additional time steps while $\begop$ is
	   fixed. Then based 
       on the updating rule of Equation~\eqref{eq:opinion-round}, 
       the expressed opinion becomes
       \begin{equation}
           \label{eq:opinion-round-2-intermediate}
       \finop^{(t+T)} = (\Lambda \Stoc)^T \finop^{(t)} + \sum_{i=0}^{T-1} (\Lambda \Stoc)^i (\ID - \Lambda) \begop. 
       \end{equation} 
   \end{lemma}
   \begin{proof}
       This follows from applying Equation~\eqref{eq:opinion-round-2} $T$ times.
   \end{proof}
  
   As a corollary we obtain that when the innate opinions
   change over time, then the final expressed opinions only depend on the
   \emph{last} vector of innate opinions.
   \begin{corollary}
      \label{corollary:opinion-model-2}
	  Assume we perform a sequence of modification on the innate opinions
	  during some finite time span and let the innate opinions after the last
	  modification be $\s$. Then final expressed opinion vector is given by:
      \begin{equation}
       \z^* = (\ID - \Lambda \Stoc)^{-1}(\ID - \Lambda) \s. 
      \end{equation}
  \end{corollary}
  \begin{proof}
      Let the $t$ be time step after which we perform the final modification to
	  the innate opinions. Then we apply Lemma~\ref{lemma:opinion-model-1} and
      it follows that $\z^{(t+T)} = (\Lambda \Stoc)^T \z^{(t)} + \sum_{i=0}^{T-1} (\Lambda \Stoc)^i (\ID - \Lambda) \s$
	  for all $T\geq0$. 
      Since the absolute value of the largest eigenvalue of $\Lambda \Stoc$ is strictly smaller than 1, 
      $\lim_{T \rightarrow \infty} (\Lambda \Stoc)^T = 0$ 
      and $\lim_{T \rightarrow \infty} \sum_{i=0}^T(\Lambda \Stoc)^i = (\ID - \Lambda \Stoc)^{-1}$. 
      It follows that
	  \begin{align*}
	  	\z^*
		= \lim_{T \rightarrow \infty} \z^{(T+t)}
		= (\ID - \Lambda \Stoc)^{-1}(\ID - \Lambda) \s.
		\quad \qedhere
	  \end{align*}
  \end{proof}

  To prove that $\z^*$ and $\zz^*$ have the same distribution, recall that we
  already argued that $\s$ and $\ss$ have the same distribution. Now observe
  that $\z^*$ and $\zz^*$ are deterministic transformations of $\s$ and $\ss$
  and by Corollary~\ref{corollary:opinion-model-2} they converge to the same
  vector for a given vector of innate opinions. This finishes the proof of the
  lemma.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:hard-computing}}
The lemma follows from the fact that our model generalizes the independent
cascade model. More concretely, suppose that $\begop = 0$, i.e., all initial
innate opinions are initialized to 0. Furthermore, suppose that we set
$\varepsilon=1$ and $\delta=1$. Then it can be seen that $\Delta \ebegop{u}=1$
for all $u \in V$ and, since $\delta=1$, all vertices have the states inactive,
ignore or spread.  Now if we set $\MasIdx{\mathcal{M}}$ to the $n \times n$
identity matrix then we observe that computing $\Exp[F(\cdot)]$ in our model is
the same as computing the influence spreading through the \emph{independent
cascade model}. Since the latter is known to be \NPhard~\cite{kempe2015maximizing} and \SPhard~\cite{chen2010scalable}, we obtain
the lemma.

\subsection{Proof of Lemma~\ref{lemma:fr-1}}
Let $I_g(S)$ be the set of all nodes that can be reached from any node of $S$ in
$g$ through a live path.  Let $\pathworld{S}{u} = 1$ if there is a live path
from any node in $S$ to $u$ in $g$ and $\pathworld{S}{u} = 0$ otherwise. Let
$\randomrrp_{g, u}$ be a RR-set of $u$ in $g$. Then $F(S)$ on $g$ can be
formulated as:

\begin{equation*}
  \begin{aligned}
&\Exp[F_g(S)] \\
&=\sum_{u,v \in V} \frac{1}{n} \IND[\pathworld{S}{u} = 1] \LinGain{u} + \IND[\pathworld{S}{u} \pathworld{S}{v} = 1] \PolGain{u}{v} \\
&= \sum_{u,v \in V} \frac{1}{n} \IND[\randomrrp_{g, u} \cap S \neq \emptyset] \LinGain{u} + \IND[\randomrrp_{g, u} \cap S \neq \emptyset, \randomrrp_{g, v} \cap S \neq \emptyset] \PolGain{u}{v}
  \end{aligned}
\end{equation*}

Now let $g$ be randomly generated possible world. We denote the distribution of
$g$ by $\c+G$ and write $g \sim \c+G$. Then we obtain:
\begin{equation}
\label{eq:bridge}
    \begin{split}
        &\Exp[F(S)] \\
		    &= \Exp_{g \sim \c+G} [\sum_{u,v \in V} (\IND[\randomrrp_{u} \cap S \neq \emptyset] \LinGain{u} + n\IND[\randomrrp_{u} \cap S \neq \emptyset, \randomrrp_{v} \cap S \neq \emptyset] \PolGain{u}{v})] \\
        &= \sum_{u,v \in V} \Exp_{g \sim \c+G} [ \IND[\randomrrp_{u} \cap S \neq \emptyset] \LinGain{u} + n\IND[\randomrrp_{u} \cap S \neq \emptyset, \randomrrp_{v} \cap S \neq \emptyset] \PolGain{u}{v}] \\
        &= n \Exp_{(u, v) \sim V^2, g \sim \c+G} \estimator \\
        &= n \Exp_{(u, v) \sim V^2, g \sim \c+G}[\frac{\sum_{(\randomrrp_u, \randomrrp_v) \in \c+R} \estimator}{\abs{\c+R}}] \\
        &= n \Exp_{(u, v) \sim V^2, g \sim \c+G}[\fracrrp{S}]
    \end{split}
\end{equation}

Thus $n\fracrrp{S}$ with sample $\c+R$ is an unbiased estimator of $\Exp[F(S)]$. 

\subsection{Proof of Lemma~\ref{lem:approximation}}
Before we prove the lemma, we first introduce martingales and some concentration
inequalities. We prove the lemma at the end of the subsection.

Let $x_1, x_2, \ldots, x_{\theta}$ be a sequence of random variables. 
For each $1\leq i \leq \theta$, we set $x_i = \estimator$.
Now observe that $\fracrrp{S} = \frac{\sum_{i=1}^\theta x_i}{\theta}$
and according to Lemma~\ref{lemma:fr-1}, $\set+E[F(S)] = \frac{n}{\theta}\cdot\set+E[\sum_{i=1}^\theta x_i]$. 
Similar to IMM~\cite{tang2015influence} and TDEM~\cite{aslay2018maximizing}, 
we determine the sample size by concentration laws of martingales. Let us first
introduce martingales. 

\begin{definition}[Martingale]
   A sequence of random variables $Y_1, Y_2, Y_3, \ldots$ 
   is a \emph{martingale} if and only if $\set+E[\abs{Y_i}] < +\infty$
   and $\set+E[Y_i \mid Y_1, Y_2, \ldots, Y_{i-1}] = Y_{i-1}$ 
   for any $i$.
\end{definition}

Note that as the generation of an \rr-set $\randomrrp_i$ is independent of $\randomrrp_1, \ldots, \randomrrp_{i-1}$, 
we have $\Exp[x_i \mid x_1, \ldots, x_{i-1}] = \frac{\Exp[F(S)]}{n^2}$. 
Now let $x = \frac{1}{n}\Exp[F(X)]$ and $M_j= \sum_{z=1}^{j}(x_z - x)$.
Then $\Exp[M_j] = 0$ and
\begin{displaymath}
 \begin{aligned}
\Exp[M_j \mid M_1, \ldots, M_{j-1}] &= \Exp[M_{j-1} + x_j - x \mid M_1, \ldots, M_{j-1}] \\
&= M_{j-1} - x + \Exp[x_j] \\
&= M_{j-1}.
\end{aligned}
\end{displaymath}
Therefore, the sequence $M_1, \ldots, M_{\theta}$ is a martingale.
Next, we restate a concentration inequality for martingales by 
McDiarmid~\cite{mcdiarmid1998concentration}, which we cite from Chung and Lu~\cite{chung2006concentration}.
\begin{lemma}[Theorem $6.1$ in~\cite{chung2006concentration}]
\label{lemmaMartIneqLiterature-1}
	Let $Y_1, Y_2, \ldots $ be a martingale,
	such that $Y_1 \le a$, $\Var[Y_1] \le b_1$, $\lvert Y_z - Y_{z-1} \rvert \le a$ for $z \in [2,j]$, and
	\[
	\Var[Y_z \mid Y_1, \ldots, Y_{z-1}] \le b_j, \text{ for } z \in [2,j],
	\]
	where $\Var[\cdot]$ denotes the variance. Then, for any $\gamma > 0$
	\begin{displaymath}
	\begin{aligned}
	\Pr(Y_j - \Exp[Y_j] \ge \gamma) \le \exp\left(-\dfrac{\gamma^2}{2(\sum_{z = 1}^{j} b_z + a \gamma /3)} \right)
	\end{aligned}
	\end{displaymath}
\end{lemma}

We now use Lemma~\ref{lemmaMartIneqLiterature-1} 
to get the concentration result for the martingale
$M_1, \ldots, M_{\theta}$.
As we define the random variables $x_i$ as $x_i = \estimator = \IND[(\randomrrp_u \cap S) \neq \emptyset] \LinGain{u}   + n\IND[(\randomrrp_u \cap S) \neq \emptyset, (\randomrrp_v \cap S) \neq \emptyset] \PolGain{u}{v}$, 
let $\chi = \max_{u, v} \abs{\LinGain{u} + n\PolGain{u}{v}}$, then $\max x_i \leq \chi$. 

Since $x_j \in [-\chi,\chi]$ for all $j \in \{1,\dots,\theta\}$,
we have $\lvert M_1 \rvert= \lvert x_1 - x \rvert \le 2\chi$ and
$\lvert M_j - M_{j-1} \rvert \le 2\chi$ for any $j \in [2,\theta]$.
Additionally, it holds that
 $\Var[M_1] = \Var[x_1]$, and for any $j \in \{2,\dots,\theta\}$ we have that:
\begin{displaymath}
 \begin{aligned}
\Var[M_j  \mid M_1, \ldots, M_{j-1}] 
&=  \Var[M_{j-1} + x_j - x \mid M_1, \ldots, M_{j-1}] \\
&=\Var[x_j \mid M_1, \ldots, M_{j-1}]  \\
&=\Var[x_j].
\end{aligned}  
\end{displaymath}

And for $\Var[x_j]$ we have that:
\begin{displaymath}
  \begin{aligned}
    \Var[x_j] &= \Exp[x_j^2] - \Exp[x_j]^2 
    \leq \chi x - x^2
    \leq \chi x.
  \end{aligned} 
\end{displaymath}

By using Lemma~\ref{lemmaMartIneqLiterature-1}, for
$M_{\theta}=  \sum_{j=1}^{\theta}(x_j - x)$, with
$\Exp[M_{\theta}] = 0$, $a = 2\chi$, $b_j=\chi x$, for $j  = 1, 2, \ldots ,\theta$, and
$\gamma = \delta \theta x$, we have the following corollary.

\begin{corollary}
\label{corr:ourIneq1}
For any $\delta > 0$,
\begin{displaymath}
\begin{aligned}
\Pr[\sum_{j=1}^{\theta} x_j - \theta x \ge \delta \theta x] \le \exp\left(-\dfrac{\delta^2}{2\chi(\frac{2\delta}{3} + 1)} \, \theta x \right).
\end{aligned}   
\end{displaymath}
\end{corollary}
Moreover, for the martingale $-M_1, \ldots, -M_{\theta}$,
we similarly have $a = 2\chi$ and $b_j = \chi x$ for $j  = 1, \ldots ,\theta$.
Note also that $\Exp[-M_{\theta}] = 0$.
Hence, %
for $-M_{\theta}=  \sum_{j=1}^{\theta}(x - x_j)$ and 
$\gamma = \delta \theta x$ we obtain a corollary similar to the one above.
\begin{corollary}\label{corr:ourIneq2}
For any $\delta > 0$,
\begin{displaymath}
\begin{aligned}
\Pr[\sum_{j=1}^{\theta} x_j - \theta x \le -\delta \theta x ] \le \exp\left(-\dfrac{\delta^2}{2\chi(\frac{2\delta}{3} + 1)} \, \theta  x \right).
\end{aligned}  
\end{displaymath}
\end{corollary}

\begin{proof}[Proof of Lemma~\ref{lem:approximation}]
Using Corollaries~\ref{corr:ourIneq1} and~\ref{corr:ourIneq2} and letting 
$\delta = \dfrac{\epsilon\, \optvalue}{2 n x}$, we obtain
   \begin{displaymath}
   \begin{aligned}
     &\Pr[\abs{n\fracrrp{X} - \Exp[F(X)]} \geq \frac{\epsilon}{2}\optvalue] \\
	 &= \Pr[\abs{\sum_{i=1}^{\theta}x_i - \theta x} {\geq \frac{\theta\epsilon}{2n}}\optvalue] \\ 
&\le 2 \exp\left(-\dfrac{\delta^2}{2\chi(\frac{2\delta}{3} + 1)} \, \theta x \right)  \\ 
& = 2 \exp\left(-\dfrac{3 \epsilon^2 \, \optvalue^2}{8\,n \chi( \epsilon\, \optvalue + 3 n x)}  \, \theta \right) \\
& \le 2 \exp\left(-\dfrac{3 \epsilon^2 \, \optvalue^2}{8\,n \chi ( \epsilon\, \optvalue + 3 \optvalue)}  \, \theta \right) \\
&= 2 \exp\left(-\dfrac{\epsilon^2 \, \optvalue}{8\,n \chi ( \frac{\epsilon}{3} + 1)}  \, \theta \right), 
   \end{aligned} 
  \end{displaymath}  
where the last inequality above follows from the fact that $n x \le \optvalue$.
Finally, by requiring
\begin{align*}
2 \exp\left(-\dfrac{\epsilon^2 \, \optvalue}{8\,n \chi ( \frac{\epsilon}{3} + 1)}  \, \theta \right)  \le \dfrac{1}{n^{\ell} \, \binom{n}{k}},
\end{align*}
we obtain the lower bound on $ \theta$.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:greedy-marketing}}
\label{sec:app-sum-index}
First, we prove that the $\fracrrp{S}$ is submodular and monontone under the 
setting of maximizing the sum of expressed opinions. Recall that we set
$$\fracrrp{S} = \frac{\sum_{\randomrrp_u \in \rrpsample} \Delta \ebegop{u} \IND[(\randomrrp_u \cap S) \neq \emptyset] }{\abs{\rrpsample}}.$$
The submodularity and monotonicity follow from the weighted version of
maximum set coverage problem, and these two properties ensure that greedy
algorithm on $\fracrrp{S}$ achieves an approximation ration of $1-\frac{1}{e}$. 
We present the details below. 

Let $S \subset T \subseteq U$, let $v \in U \setminus T$.

First, we show that $\fracrrp{S}$ is monontone: Since for any $R_u \in \rrpsample$, $\IND[(\randomrrp_u \cap T) \neq \emptyset] - \IND[(\randomrrp_u \cap S) \neq \emptyset] \geq 0$, 
thus, $\fracrrp{T} - \fracrrp{S} \geq 0$. 

Second, we show that $\fracrrp{S}$ is submodular: Since for any $R_u \in \rrpsample$, 
$(\IND[(\randomrrp_u \cap (T\cup\{v\})) \neq \emptyset] - \IND[(\randomrrp_u \cap T) \neq \emptyset]) \leq (\IND[(\randomrrp_u \cap (S\cup\{v\})) \neq \emptyset] - \IND[(\randomrrp_u \cap S) \neq \emptyset])$, 
thus, $\fracrrp{T \cup \{v\}} - \fracrrp{T} - (\fracrrp{S \cup \{v\}} - \fracrrp{S}) \leq 0$. 

Now we apply Lemma~\ref{lem:y-size-main} and Lemma~\ref{lem:approximation} to
obtain a lower bound on $\optvalue$ and the sampling size $\theta$. This ensures that
Equation~\eqref{equation:sample-error-bound} holds.

Note that there are in total $\binom{n}{k}$ different sets of size $k$ and thus
there are $\binom{n}{k}$ ways to choose $S$. Applying a union bound to
Equation~\eqref{equation:sample-error-bound}, we obtain that
   \[\set+P[\abs{n\cdot \fracrrp{S} - \Exp[F(S)]} \geq \frac{\epsilon}{2}\cdot \optvalue \mid \mbox{for any $S$ of size k}] \leq \frac{1}{n^{\ell}}.\]

   Let $S^{G}$ denote the greedy solution for $F_{\c+R}(\cdot)$, 
   $S^{+}$ the optimal solution for $F_{\c+R}(\cdot)$, 
   and $S^*$ the optimal solution for $\Exp[F(\cdot)]$.
   Then the following inequality holds with probability at least $1 - n^{-\ell}$:
   \begin{equation*}
      \begin{aligned}
         \Exp[F(S^G)] &\geq n \fracrrp{S^G} - \frac{\epsilon}{2} \optvalue \\
         &\geq n (1 - \frac{1}{e}) \fracrrp{S^+} - \frac{\epsilon}{2} \optvalue \\
         &\geq n (1 - \frac{1}{e}) \fracrrp{S^*} - \frac{\epsilon}{2} \optvalue \\
         &\geq (1 - \frac{1}{e}) (\Exp[F(S^*)] - \frac{\epsilon}{2}\optvalue) - \frac{\epsilon}{2} \optvalue \\
         &= (1 - \frac{1}{e})\optvalue - (1 - \frac{1}{e}) \frac{\epsilon}{2} \optvalue - \frac{\epsilon}{2} \optvalue \\
         &\geq (1 - \frac{1}{e} - \epsilon) \optvalue.
      \end{aligned}
   \end{equation*}
Thus implementing the greedy algorithm on $F_{\c+R}(\cdot)$ directly gives us a
$(1 - \frac{1}{e} - \epsilon)$-approximation with high probability. 
	
\subsection{Proof of Lemma~\ref{lemma:max-sum-opinions}}
It is well-known that for the Laplacian $\laplacian$ of undirected graphs it
holds that $\ind^\intercal (\ID + \laplacian)^{-1} = \ind^{\intercal}$.
Now we obtain:
\begin{equation}
  \begin{aligned}
	\arg\max_S \sum_{u \in V} \efinop{u}^*(S)
		&= \arg \max_{S} \ind^\intercal [(\ID + \laplacian)^{-1} (\begop + \Delta \begop \odot \ind(S))]\\
		&=  \arg \max_{S} \ind^\intercal [\Delta \begop \odot \ind(S)] \\
		&=  \arg \max_{S} \sum_{u \in V} \Delta \ebegop{u} \ind_u(S) \\
		&= \arg\max_S F(S).
  \end{aligned}
\end{equation}

\subsection{Proof of Lemma~\ref{lemma:approx-max-sum-opinions}}
  Let $S \subset T \subseteq U$, let $v \in U \setminus T$. 
We first prove that in any possible world $g$, $F_g(S)$ is submodular and monontone.

First, we show that $F_g(S)$ is monontone: Since for any $u \in V$, 
  $\ind_u(T) - \ind_u(S) \geq 0$, 
thus, $F_g(T) - F_g(S) \geq 0$. 

Second, we show that $F_g(S)$ is submodular: Since for any $u \in V$, 
$\ind_u(T\cup\{v\})- \ind_u(T) \leq \ind_u(S\cup\{v\})- \ind_u(S)$, 
thus, $F_g(T \cup \{v\}) - F_g(T) - (F_g(S \cup \{v\}) - F_g(S)) \leq 0$. 

Now $\Exp[F(S)]$ is submodular and monontone as it is a linear combination of
the $F_g(S)$, and the weight for each part is non-negative. 
The approximation ratio of greedy algorithm on $\Exp[F(S)]$ is thus
$1 - \frac{1}{e}$~\cite{hochbaum1996approximating}.

\subsection{Proof of Lemma~\ref{lem:y-size-main}}
\emph{Proof of~(1).}
Let $X$ be a
set of seed nodes with 
$\abs{X} = k$ and let $x = \frac{1}{n} \Exp[F(X)]$.
We show that if $\opt < y\chi$ then
$n\fracrrp{X} \geq (1 + \epsilon_2) \,y \chi$
with probability at most $\frac{n^{-\ell}}{\log_2 n \binom{n}{k}}$.  

Note that $\optvalue < y \chi$ implies that $x < \frac{\opt}{n} < \frac{y \chi}{n}$,
and $1 < \frac{y \chi}{xn}$. Notice that by construction $y \leq n$ since in the
algorithm we set $y \leftarrow n/2^i$. 
Let $\delta = \frac{1 + \epsilon_2}{n x} y \chi - 1$ and observe that
$\delta > \frac{\epsilon_2 y \chi}{n x}$. 
Then, by using Corollary~\ref{corr:ourIneq1}, we have:
  \begin{displaymath}
    \begin{aligned}
      \Pr[n\fracrrp{X} \geq (1 + \epsilon_2)y] &= \Pr\left[\theta \fracrrp X - \theta x \geq \theta x \left(\frac{(1 + \epsilon_2)y\chi}{nx} - 1\right)\right] \\
      &= \Pr[\theta \fracrrp X - \theta x \geq \theta x \delta] \\  
      &\leq \exp \left(-\frac{\delta}{2 \chi (\frac{2}{3} + \frac{1}{\delta})}\theta x\right) \\
      &\leq \exp \left(-\frac{\delta}{2 \chi (\frac{2}{3} + \frac{1}{\epsilon_2})}\theta x\right) \\
      &\leq \exp \left(-\frac{\epsilon_2^2}{\frac{4}{3}\epsilon_2 + 2}\frac{y}{n}\theta\right) \\
      &\leq \frac{n^{-\ell}}{\log_2(n)\cdot \binom{n}{k}}.
    \end{aligned}
  \end{displaymath}
Finally by a union bound over all $\binom{n}{k}$ choices of $X$, we conclude
that if $\opt < y \chi$, then $n\fracrrp{\t+X} < (1 + \epsilon_2)y$ with
probability at least $1 - \frac{n^{-\ell}}{\log_2 n}$.

\emph{Proof of~(2).}
  Let $X$ be a set of seed nodes with $\abs{X} = k$ and let $x = \frac{1}{n} \Exp[F(X)]$.
  Assume that 
  $\opt \geq y\chi$. Note that this implies $\frac{\optvalue}{nx} \geq 1$.
  Now we will show that if $\opt \geq y \chi$ then $n \, \fracrrp{\t+X} > (1 + \epsilon_2)\optvalue$
  with probability at most $\frac{n^{-\ell}}{\log_2 n \binom{n}{k}}$. 

  Let $\delta = \frac{(1 + \epsilon_2) \optvalue}{n x} - 1$. Then we have $\delta \geq \epsilon_2$. 
  By using Corollary~\ref{corr:ourIneq2}, we obtain that:
  \begin{displaymath}
    \begin{aligned}
      &\Pr[n \, \fracrrp{X} > (1 + \epsilon_2)\opt] \\
	  &= \Pr\left[\theta \fracrrp X - \theta x > \theta x \left(\frac{(1 + \epsilon_2)\opt}{nx} - 1\right)\right] \\
      &\leq \exp \left(-\frac{\delta}{2 \chi (\frac{2}{3} + \frac{1}{\delta})}\theta x\right) \\
      &\leq \exp \left(-\frac{\delta}{2 \chi (\frac{2}{3} + \frac{1}{\epsilon_2})}\theta x\right) \\
      &\leq \exp \left(-\frac{\epsilon_2 \optvalue}{2 \chi n (\frac{2}{3} + \frac{1}{\epsilon_2})}\theta \right) \\
      &\leq \exp\left(-\frac{\epsilon_2^2}{\frac{4}{3}\epsilon_2 + 2}\frac{y}{n}\theta\right) \\
      &\leq \frac{n^{-\ell}}{\log_2(n) \cdot \binom{n}{k}}
    \end{aligned}
  \end{displaymath}
By taking a union bound over all $\binom{n}{k}$ choices of $X$, we reach the
desired result.

\subsection{Proof of Theorem~\ref{theorem:sand-lu}}
Our proof has four steps. 
First, we show that the matrices $\MasIdx{\ConIdx{}}$ and
$\MasIdx{\DisConIdx{}}$ have non-negative entries.
Second, we show that 
the objective function $\mu_0(S)$ is monotone but neither submodular nor supermodular.
Third, we show that the upper and lower bounds we consider are monotone and submodular.
Fourth, we apply the sandwich method.

\emph{Step~I: The matrices $\MasIdx{\ConIdx{}}$ and $\MasIdx{\DisConIdx{}}$ have
	non-negative entries.}
As we defined in Table~\ref{table:index}, 
$\MasIdx{\ConIdx{}} = (\laplacian + \ID)^{-2}$
and $\MasIdx{\DisConIdx{}} = (\laplacian + \ID)^{-1}$. 
We now show that all entries of $\MasIdx{\DisConIdx{}}$ 
are non-negative. Note that this implies that the entries of
$\MasIdx{\ConIdx{}}$ are non-negative as well since 
$\MasIdx{\ConIdx{}} = \MasIdx{\DisConIdx{}}^2$. 

Now observe that:
\begin{equation*}
  \begin{aligned}
    (\laplacian + \ID)^{-1} &= [(\m+D + \ID) (\ID - (\ID + \m+D)^{-1} \m+W)]^{-1} \\
    &=(\ID - (\ID + \m+D)^{-1} \m+W)^{-1}(\m+D + \ID)^{-1} \\
    &=[\sum_{i=0}^{\infty} (\ID + \m+D)^{-i}\m+W^i] (\m+D + \ID)^{-1}.
  \end{aligned}
\end{equation*}
The last equation holds since the entries of matrix $(\ID + \m+D)^{-1} \m+W$ are non-negative, and 
the sum of rows and columns are strictly smaller than 1, thus the limit $\lim_{i\rightarrow \infty} (\ID + \m+D)^{-i} \m+W^i = 0$.  
As each matrix $(\ID + \m+D)^{-i}\m+W^i$, and $(\m+D + \ID)^{-1}$ 
are non-negative, their sums and multiplication are non-negative. 
Thus $(\laplacian + \ID)^{-1}$ is non-negative. 

\emph{Step~II: The objective function $\mu_0(S)$ is monotone but neither submodular nor supermodular.}
Let $\MasIdx{\mathcal{M}} \in \{ \MasIdx{\DisConIdx{}}, \MasIdx{\ConIdx{}} \}$, 
our goal is to maximize $\Exp[\s^{\intercal} \MasIdx{\c+M} \s]$ 
by selecting a set of seed nodes $S$. 
Let
$$\mu_0(S) = \Exp[2 \begop^\intercal \MasIdx{\mathcal{M}} \Delta \s + \Delta \s^\intercal \MasIdx{\mathcal{M}} \Delta \s].$$
By substituting $\s=\begop+\Delta\s$ into $\Exp[\s^{\intercal} \MasIdx{\c+M}
\s]$ and ignoring summands which only depends on $\begop$, we have 
$$\arg \max_S \mu_0(S) = \arg \max_S \Exp[\s^{\intercal} \MasIdx{\c+M} \s].$$

Now, we show that $\mu_0(S)$ is neither submodular nor supermodular, 
but monontone in the following Lemma~\ref{lem:non-sub-super}, and Lemma~\ref{lem:mon}. 

\begin{lemma}
  \label{lem:non-sub-super}
  $\mu_0(S)$ is neither submodular nor supermodular.
\end{lemma}
\begin{proof}
$\mu_0(S)$ is not submodular:
We can set the spread probabilities $p_{uv}$ on
all the edges to be $0$, and $\delta = 0$ as well. 
We also set the non-adjusted innate opinions 
$\begop = \m+0$. In this case, $\mu_0(S)$ becomes
$\mu_0(S) = \Exp[\Delta \s^{\intercal} \MasIdx{\mathcal{M}} \Delta \s] = \sum_{u \in S, v \in S} \Delta \ebegop{u} \Delta \ebegop{v} \MasIdx{\mathcal{M}}_{u,v}$.
As in Sec.~\ref{sec:estimating}, we set $m_{u, v} = (\Delta \ebegop{u})^{\intercal} \MasIdx{\mathcal{M}}_{u,v} \Delta \ebegop{v}$. 
Let $S \subseteq T \subseteq U$, and $x \in U \setminus T$, 
$\mu_0(T \cup \{x\}) - \mu_0(T) - (\mu_0(S \cup \{x\}) - \mu_0(S)) = \sum_{u \in T \setminus S} m_{u, x} + \sum_{v \in T \setminus S} m_{x, v} \geq 0$.
The inequality is strict $>$ if any $m_{u, x}$ or $m_{x, v}$, $u, v \in T \setminus S$
is strictly larger than 0. This condition can be satisfied by selecting $v$. 

$\mu_0(S)$ is not supermodular:
We set non-adjusted innate opinions $\begop = \m+0$, 
and $\epsilon$ small enough such that $\Delta \ebegop{u} = \epsilon$ for any $u$. 
We set $w_{uv} = 0$ for any $(u, v) \in E$. 
In addition, we set $\delta = 1$, such that \spread becomes independent cascade model. 
Under these settings, 
$\MasIdx{\mathcal{M}}$ is the identity matrix $\ID$, and 
$\mu_0(S) = \epsilon^2 \sum_{v \in V} \ind_u(S)$. 
Note that $\sum_{u\in V}\ind_u(S)$ is the influence spread in the independent
cascade model with seed set $S$, 
which is submodular~\cite{kempe2015maximizing}. 
Let $\sigma(S) = \sum_{u\in V}\ind_u(S)$. 
Let $S \subseteq T \subseteq U$, and $x \in U \setminus T$, 
from the submodularity of $\sigma(S)$ it follows 
$\mu_0(T \cup \{x\}) - \mu_0(T) - (\mu_0(S \cup \{x\}) - \mu_0(S)) = 
\epsilon^2 \sum_{u \in V} (\sigma(T \cup \{x\}) - \sigma(T)) - (\sigma(S \cup \{x\}) - \sigma(S)) \leq 0$.
Now, let $S = \emptyset$, and select $T$ and $\{x\}$ such that $\sigma(T) =
\abs{V}$ and $\sigma(\{x\}) > 0$.
The inequality is strict. 
\end{proof}

\begin{lemma}
  \label{lem:mon}
  $\mu_0(S)$ is monontone.
\end{lemma}
\begin{proof}
  Let $S \subseteq T$. Then
  $$\mu_0(T) - \mu_0(S) = \sum_{u, v \in V} m_{u, v} (\ind_{u}(T) \ind_{v}(T) - \ind_{u}(S) \ind_{v}(S)) \geq 0$$
  since $\ind_{v}(T) \geq \ind_{v}(S)$ for any $v \in V$. 
\end{proof}

\emph{Step~III: The upper and lower bound are monotone and submodular.}
For 
$\mu_L(S) = \Exp[2 \begop^\intercal \MasIdx{\mathcal{M}} \Delta \s]$, 
$\mu_U(S) = \Exp[2 \begop^\intercal \MasIdx{\mathcal{M}} \Delta \s + \Delta \s^\intercal \MasIdx{\mathcal{M}}^U \Delta \s]$,
we prove that both $\mu_L(S)$ and $\mu_U(S)$ are submodular. 

\begin{lemma}
  \label{lem:sub-two}
  $\mu_L(S)$ and $\mu_U(S)$ are submodular. 
\end{lemma}
\begin{proof}
  We use the notation defined in Sec.~\ref{sec:estimating}, i.e., we set
$\LinGain{u} = (2\begop^\intercal \MasIdx{\mathcal{M}})_u \Delta \ebegop{u}$ and
$\PolGain{u}{v}=(\Delta \ebegop{u})^\intercal \MasIdx{\mathcal{M}}_{u,v} \Delta
\ebegop{v}$. 
Then, $\mu_L(S) = \sum_u \LinGain{u} \ind_u(S)$, and $\mu_U(S) = \sum_u (\LinGain{u} + \sum_{v\in V}\MasIdx{\mathcal{M}}_{u,v}\Delta \ebegop{u}^2) \ind_{u}(S)$. 
Let $S \subseteq T \subseteq U$, and $x \in U \setminus T$, since 
for any $u \in V$, 
$\ind_u(S \cup \{x\}) - \ind_u(S) \geq \ind_u(T \cup \{x\}) - \ind_u(T)$, 
and the weight $\LinGain{u}$, $(\LinGain{u} + \sum_{v\in V}\MasIdx{\mathcal{M}}_{u,v}\Delta \ebegop{u}^2)$ are positive. 
We have $\mu_L(S \cup \{x\}) - \mu_L(S) \geq \mu_L(T \cup \{x\}) - \mu_L(T)$ and 
$\mu_U(S \cup \{x\}) - \mu_U(S) \geq \mu_U(T \cup \{x\}) - \mu_U(T)$. 
It follows that $\mu_L(S)$ and $\mu_U(S)$ are submodular. 
\end{proof}

\emph{Step~IV: Application of the sandwich method.}
Similarly with Lemma~\ref{lem:mon}, we can also see that $\mu_L(S)$ 
and $\mu_U(S)$ are monotone. 
Since $\mu_0(S)$ is monotone, and both $\mu_L(S)$ and $\mu_U(S)$ are submodular and monontone, 
we can apply the sandwich approximation scheme proposed by Lu et al.~\cite[Theorem 9]{lu2015competition},
and it gives us the approximation result.  



==> arXiv version/tables/backfire-2.tex <==
\begin{table*}[!htb]
\caption{Results for polarizing campaigns with
	$k = \lceil 0.5\%\cdot n\rceil$ seeds,
	where we initialized the innate opinions using the uniform distribution.
	We report the relative increase of each index in percent.}
\label{tab:backfire-2}
\centering
  \vspace{-4mm}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c ccccccccc ccccccccc}
\toprule
\textbf{Dataset}  & \multicolumn{9}{c}{\textbf{\disidx}} & \multicolumn{9}{c}{\textbf{\intidx}} \\
\cmidrule(lr){2-10} 
\cmidrule(lr){11-19} 
 & \MaxSum & \MaxLinDisCon & \MaxLinPol & \MaxLinDis & \MaxLinInt &  \MaxInfluence & \Random & \FJGreedy & \FJUpp & \MaxSum & \MaxLinDisCon & \MaxLinPol & \MaxLinDis & \MaxLinInt &  \MaxInfluence & \Random & \FJGreedy &\FJUpp\\
\midrule
\Netscience  & 3.64 & 5.36 & 2.31 & \textbf{7.33} & \textbf{7.33} & 7.32 & 0.68 & 1.04 &  15.84   & 4.85 & 4.88 & 0.97 & 7.41 & 7.95 & \textbf{7.96} & 0.68 & 1.1 &  16.98   \\
\WikiVote  & 2.6 & 5.79 & 11.05 & \textbf{11.09} & 10.93 & \textbf{11.09} & 0.68 & 1.12 &  15.74   & 2.26 & 6.06 & 12.36 & 12.41 & 12.6 & \textbf{12.68} & 0.67 & 1.17 &  17.84   \\
\Reed  & 5.62 & 5.55 & 6.01 & \textbf{8.89} & 8.4 & 8.39 & 0.73 & 2.74 &  44.57   & 5.98 & 5.31 & 1.99 & 7.96 & \textbf{8.49} & 8.48 & 0.71 & 0.77 &  11.49   \\
\EmailUniv  & 2.69 & 4.63 & 7.7 & \textbf{8.2} & 8.15 & 8.11 & 0.79 & 1.32 &  19.14   & 2.29 & 4.43 & 8.9 & \textbf{9.94} & 9.88 & 9.84 & 0.78 & 1.0 &  14.67   \\
\Hamster  & 3.25 & 4.96 & 7.61 & \textbf{10.08} & 10.02 & 10.06 & 0.68 & 1.45 &  22.82   & 3.1 & 5.01 & 7.49 & 11.15 & 11.42 & \textbf{11.48} & 0.65 & 0.84 &  12.85   \\
\USFCA  & 2.74 & 4.02 & 5.58 & \textbf{7.17} & 6.83 & 6.87 & 0.79 & 3.2 &  50.80   & 1.83 & 2.51 & 3.92 & 8.16 & 8.67 & \textbf{8.7} & 0.77 & 0.8 &  11.81   \\
\NipsEgo  & 37.94 & 59.44 & 59.44 & 59.44 & \textbf{59.45} & 59.44 & 0.46 & 0.71 &  10.22   & 37.32 & 58.95 & 58.93 & 58.95 & \textbf{58.96} & 58.94 & 0.46 & 1.54 &  39.06   \\
\PagesGovernment  & 3.41 & 4.61 & 7.52 & \textbf{9.28} & 7.83 & 8.48 & 0.69 & 1.83 &  29.07   & 2.48 & 3.86 & 6.05 & 9.05 & \textbf{10.09} & 9.99 & 0.7 & 0.83 &  12.67   \\
\HepPh  & 2.36 & 3.49 & 4.82 & \textbf{6.46} & 5.53 & 5.97 & 0.68 & 1.24 &  18.85   & 1.58 & 2.58 & 4.14 & 6.79 & \textbf{7.51} & 7.36 & 0.7 & 0.98 &  14.81   \\
\Anybeat  & 27.84 & 36.77 & 38.55 & \textbf{38.58} & 38.19 & 38.5 & 0.5 & 0.85 &  12.63   & 22.18 & 30.28 & 31.73 & 32.13 & \textbf{32.56} & 32.35 & 0.55 & 1.37 &  22.25   \\
\CondMat  & 3.04 & 4.7 & 5.39 & \textbf{7.31} & 6.76 & 7.05 & 0.65 & 1.15 &  17.84   & 2.71 & 4.61 & 4.77 & 7.92 & \textbf{8.46} & 8.35 & 0.65 & 0.98 &  15.40   \\
\Gplus  & 28.44 & 56.09 & 56.51 & \textbf{56.52} & 56.51 & 56.51 & 0.66 & 0.72 &  10.73   & 25.87 & 53.11 & 53.61 & 53.62 & \textbf{53.64} & 53.63 & 0.66 & 1.53 &  29.31   \\
\Brightkite  & 5.4 & 14.28 & 16.85 & \textbf{17.13} & 16.81 & 17.12 & 0.7 & - &  -   & 5.28 & 15.41 & 17.73 & 18.33 & 18.55 & \textbf{18.56} & 0.69 & - &  -   \\
\WikiTalk  & 13.15 & 25.45 & 28.31 & \textbf{28.32} & 27.97 & 28.26 & 0.74 & - &  -   & 12.09 & 23.02 & 25.35 & 25.51 & \textbf{25.69} & \textbf{25.69} & 0.74 & - &  -   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}



==> arXiv version/tables/backfire-short.tex <==
\begin{table*}[ht!]
\caption{Results for polarizing campaigns with
	$k = \lceil 0.5\%\cdot n\rceil$ seeds.
	We report the relative increase of each index in percent.}
\label{tab:backfire}
\centering
  \vspace{-4mm}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c ccccccccc ccccccccc}
\toprule
\textbf{Dataset}  & \multicolumn{8}{c}{\textbf{\sumidx}} & \multicolumn{9}{c}{\textbf{\polidx}} \\
\cmidrule(lr){2-9} 
\cmidrule(lr){10-18} 
  &  \MaxSum  &  \MaxLinDisCon  &  \MaxLinPol  &  \MaxLinDis  &  \MaxLinInt  &   \MaxInfluence  &  \Random  &  \FJGreedy  &  \MaxSum  &  \MaxLinDisCon  &  \MaxLinPol  &  \MaxLinDis  &  \MaxLinInt  &  \MaxInfluence  &  \Random  & \FJGreedy  & \FJUpp \\
\midrule
\Netscience   & \textbf{0.48} & 0.46 & 0.04 & 0.07 & 0.34 & 0.34 & -0.01 & 0.11  & 2.72 & 5.03 & \textbf{7.62} & 5.54 & 5.65 & 5.66 & 0.62 & 2.36 &   10.54   \\
\WikiVote   & \textbf{0.33} & 0.25 & -0.28 & -0.28 & -0.27 & -0.33 & -0.02 & 0.11  & 3.14 & 5.83 & 9.46 & \textbf{9.5} & 9.09 & 9.14 & 0.64 & 2.92 &   12.29   \\
\Reed   & \textbf{0.27} & \textbf{0.27} & 0.02 & 0.18 & 0.16 & 0.16 & 0.01 & 0.1  & 6.6 & 7.68 & \textbf{15.82} & 11.35 & 8.87 & 8.79 & 0.74 & 9.56 &   68.48   \\
\EmailUniv   & \textbf{0.33} & 0.31 & -0.23 & -0.21 & -0.18 & -0.16 & -0.02 & 0.11  & 3.39 & 5.23 & \textbf{7.72} & 7.36 & 6.87 & 6.81 & 0.79 & 3.8 &   18.12   \\
\Hamster   & \textbf{0.3} & 0.27 & -0.07 & -0.09 & -0.11 & -0.1 & -0.01 & 0.1  & 4.3 & 5.2 & \textbf{11.1} & 8.98 & 8.55 & 8.56 & 0.66 & 5.18 &   25.70   \\
\USFCA   & \textbf{0.22} & \textbf{0.22} & 0.05 & -0.04 & -0.02 & -0.02 & -0.01 & 0.11  & 6.85 & 10.05 & \textbf{13.18} & 7.39 & 5.68 & 5.74 & 0.74 & 11.57 &   82.48   \\
\NipsEgo   & \textbf{0.46} & 0.22 & 0.2 & 0.21 & 0.21 & 0.21 & 0.0 & 0.1  & 38.05 & 59.55 & \textbf{59.57} & 59.56 & 59.55 & \textbf{59.57} & 0.46 & 0.79 &   5.34   \\
\PagesGovernment   & \textbf{0.29} & 0.28 & -0.03 & 0.01 & 0.0 & -0.0 & -0.0 & 0.1  & 4.78 & 5.89 & \textbf{12.73} & 10.1 & 6.19 & 7.48 & 0.66 & 6.96 &   36.87   \\
\HepPh   & \textbf{0.33} & 0.32 & -0.01 & -0.08 & -0.1 & -0.1 & -0.01 & 0.1  & 3.69 & 5.17 & \textbf{7.62} & 5.91 & 4.61 & 5.16 & 0.66 & 3.26 &   16.03   \\
\Anybeat   & \textbf{0.42} & 0.3 & 0.11 & 0.12 & 0.14 & 0.12 & 0.0 & 0.1  & 29.3 & 38.14 & \textbf{39.84} & 39.75 & 39.12 & 39.55 & 0.48 & 1.7 &   7.80   \\
\CondMat   & \textbf{0.36} & 0.32 & 0.01 & 0.01 & 0.02 & 0.02 & 0.0 & 0.1  & 4.26 & 5.58 & \textbf{8.28} & 6.68 & 5.32 & 5.84 & 0.65 & 3.42 &   15.69   \\
\Gplus   & \textbf{0.49} & 0.15 & 0.1 & 0.1 & 0.1 & 0.1 & 0.0 & 0.1  & 29.75 & 57.48 & \textbf{57.94} & \textbf{57.94} & 57.92 & 57.93 & 0.66 & 0.92 &   6.41   \\
\Brightkite   & \textbf{0.38} & 0.24 & -0.02 & -0.0 & 0.0 & 0.01 & 0.0 & -  & 5.66 & 13.35 & \textbf{15.86} & 15.65 & 15.17 & 15.58 & 0.7 & - &   -   \\
\WikiTalk   & \textbf{0.49} & 0.29 & 0.02 & 0.01 & 0.02 & 0.02 & 0.0 & -  & 13.46 & 25.84 & \textbf{28.79} & 28.71 & 28.19 & 28.57 & 0.73 & - &   -   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> arXiv version/tables/exp-backfire-1.tex <==
\begin{table*}[ht!]
    \caption{Results for polarizing campaigns with
        $k = \lceil 0.5\%\cdot n\rceil$ seeds,
		where we initialized the innate opinions using the exponential distribution.
        We report the relative increase of each index in percent.}
    \label{tab:exp-backfire-1}
    \centering
      \vspace{-4mm}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c ccccccccc ccccccccc}
    \toprule
    \textbf{Dataset}  & \multicolumn{8}{c}{\textbf{\sumidx}} & \multicolumn{9}{c}{\textbf{\polidx}} \\
    \cmidrule(lr){2-9} 
    \cmidrule(lr){10-18} 
      &  \MaxSum  &  \MaxLinDisCon  &  \MaxLinPol  &  \MaxLinDis  &  \MaxLinInt  &   \MaxInfluence  &  \Random  &  \FJGreedy  &  \MaxSum  &  \MaxLinDisCon  &  \MaxLinPol  &  \MaxLinDis  &  \MaxLinInt  &  \MaxInfluence  &  \Random  & \FJGreedy  & \FJUpp \\
    \midrule
\Netscience  & \textbf{0.25} & \textbf{0.25} & -4.41 & -0.87 & -0.78 & -6.38 & -0.69 & \textbf{0.25} & 6.15 & 5.23 & \textbf{55.56} & 2.36 & 0.22 & 37.64 & 1.09 & 7.29 & 86.98  \\
\WikiVote  & \textbf{0.22} & 0.2 & -4.29 & -5.89 & -5.6 & -6.61 & -0.47 & 0.2 & 4.14 & 4.54 & \textbf{20.63} & 18.64 & 12.48 & 16.93 & 0.97 & 8.58 & 55.66  \\
\Reed  & 0.16 & \textbf{0.22} & -1.45 & -4.22 & -3.8 & -6.54 & -0.63 & \textbf{0.22} & 13.78 & 31.35 & \textbf{48.24} & 40.63 & 4.75 & 15.32 & 0.98 & 37.93 & 523.59  \\
\EmailUniv  & \textbf{0.21} & 0.2 & -3.39 & -5.22 & -5.19 & -5.98 & -0.51 & \textbf{0.21} & 2.2 & 6.87 & \textbf{13.28} & 11.62 & 8.31 & 9.79 & 0.8 & 11.44 & 68.31  \\
\Hamster  & 0.16 & 0.22 & -3.99 & -4.93 & -5.5 & -9.94 & -0.67 & \textbf{0.24} & 6.33 & 9.34 & \textbf{26.65} & 17.36 & 4.95 & 8.54 & 0.51 & 20.54 & 189.96  \\
\USFCA  & 0.14 & 0.19 & -0.91 & -2.8 & -4.3 & -5.39 & -0.48 & \textbf{0.2} & 6.65 & 13.99 & 28.37 & 23.41 & 9.95 & 8.48 & 0.71 & \textbf{29.95} & 396.04  \\
\NipsEgo  & \textbf{0.28} & \textbf{0.28} & -36.7 & -50.13 & -52.0 & -52.77 & -0.87 & \textbf{0.28} & 4.92 & 5.46 & \textbf{96.9} & 42.55 & 31.68 & 26.4 & 0.4 & 6.02 & 50.36  \\
\PagesGovernment  & 0.21 & 0.21 & -1.75 & -4.31 & -4.71 & -7.91 & -0.57 & \textbf{0.23} & 4.83 & 7.74 & \textbf{39.47} & 19.14 & 5.08 & 9.72 & 0.49 & 20.98 & 265.14  \\
\HepPh  & 0.17 & 0.18 & -1.8 & -2.87 & -2.53 & -7.72 & -0.81 & \textbf{0.31} & 5.94 & 6.19 & \textbf{32.43} & 18.04 & 2.7 & 10.21 & 0.18 & 20.14 & 202.7  \\
\Anybeat  & 0.28 & 0.29 & -30.31 & -30.03 & -29.7 & -36.32 & -1.01 & \textbf{0.3} & 6.46 & 7.93 & \textbf{55.25} & 50.77 & 48.3 & 39.56 & 0.27 & 11.02 & 89.58  \\
\CondMat  & 0.24 & 0.24 & -2.16 & -2.53 & -3.23 & -7.68 & -0.69 & \textbf{0.27} & 6.59 & 7.72 & \textbf{28.5} & 12.83 & 4.5 & 10.99 & 0.36 & 15.87 & 149.43  \\
\Gplus  & 0.3 & 0.31 & -26.97 & -41.32 & -38.25 & -57.37 & -0.79 & \textbf{0.32} & 7.53 & 8.02 & \textbf{120.0} & 74.17 & 70.28 & 16.68 & 0.2 & 8.97 & 79.93  \\
\Brightkite  & \textbf{0.24} & 0.23 & -9.12 & -11.47 & -10.31 & -19.24 & -0.84 &  \_ & 7.8 & 7.82 & \textbf{25.63} & 20.59 & 12.29 & 19.4 & 0.17 &  - &  -  \\
\WikiTalk  & \textbf{0.38} & \textbf{0.38} & -22.0 & -21.52 & -21.37 & -29.75 & -0.66 &  \_ & 7.23 & 8.11 & \textbf{60.33} & 51.67 & 51.64 & 47.0 & 0.76 &  - &  -  \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \end{table*}


==> arXiv version/tables/exp-backfire-2.tex <==
\begin{table*}[!htb]
    \caption{Results for polarizing campaigns with
        $k = \lceil 0.5\%\cdot n\rceil$ seeds,
		where we initialized the innate opinions using the exponential distribution.
        We report the relative increase of each index in percent.
        }
    \label{tab:exp-backfire-2}
    \centering
      \vspace{-4mm}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c ccccccccc ccccccccc}
    \toprule
    \textbf{Dataset}  & \multicolumn{9}{c}{\textbf{\disidx}} & \multicolumn{9}{c}{\textbf{\intidx}} \\
    \cmidrule(lr){2-10} 
    \cmidrule(lr){11-19} 
     & \MaxSum & \MaxLinDisCon & \MaxLinPol & \MaxLinDis & \MaxLinInt &  \MaxInfluence & \Random & \FJGreedy & \FJUpp & \MaxSum & \MaxLinDisCon & \MaxLinPol & \MaxLinDis & \MaxLinInt &  \MaxInfluence & \Random & \FJGreedy &\FJUpp\\
    \midrule
\Netscience  & 0.58 & 0.61 & \textbf{5.38} & 5.24 & 3.1 & 0.51 & -0.03 & 5.24 & 53.49 & -1.19 & -1.21 & -1.97 & 1.92 & \textbf{4.27} & -1.2 & -0.06 & 7.69 & 43.62  \\
\WikiVote  & 1.23 & 1.18 & 7.49 & \textbf{7.64} & 1.72 & 1.29 & -0.12 & 5.79 & 40.77 & 0.42 & 0.44 & 2.16 & 2.48 & \textbf{4.47} & 0.34 & -0.12 & 5.85 & 45.9  \\
\Reed  & 1.55 & 1.38 & 9.3 & 10.3 & 1.46 & 1.52 & 0.06 & \textbf{11.82} & 124.5 & 1.14 & 1.0 & 0.73 & 1.17 & \textbf{3.44} & 1.02 & 0.09 & 4.7 & 30.48  \\
\EmailUniv  & -0.37 & -0.49 & 4.41 & 5.89 & 2.58 & 0.1 & 0.02 & \textbf{6.15} & 39.9 & 0.07 & -0.15 & 0.78 & 2.08 & \textbf{4.66} & 0.34 & 0.05 & 4.82 & 37.14  \\
\Hamster  & 3.9 & 4.27 & 8.49 & \textbf{9.7} & 4.57 & 3.9 & -0.0 & 8.7 & 69.09 & 1.54 & 1.78 & 1.75 & 2.69 & \textbf{4.43} & 1.54 & -0.06 & 5.89 & 42.2  \\
\USFCA  & 0.01 & 0.2 & 10.18 & \textbf{11.36} & 2.01 & 0.03 & 0.0 & 11.18 & 123.72 & -0.03 & 0.01 & 1.03 & 1.63 & \textbf{3.14} & 0.05 & -0.02 & 4.26 & 29.82  \\
\NipsEgo  & -0.4 & -0.47 & 4.25 & \textbf{7.45} & 4.0 & -0.54 & 0.03 & 5.95 & 34.55 & -0.11 & -0.24 & 2.81 & \textbf{5.62} & 3.07 & -0.39 & 0.03 & 6.7 & 132.74  \\
\PagesGovernment  & 3.58 & 4.26 & \textbf{9.43} & 9.22 & 3.41 & 3.84 & 0.01 & 8.88 & 83.73 & 1.05 & 1.16 & 1.58 & 2.9 & \textbf{4.22} & 1.12 & 0.01 & 5.46 & 38.0  \\
\HepPh  & 5.54 & 6.13 & 10.95 & \textbf{12.25} & 5.33 & 5.93 & 0.02 & 10.26 & 77.54 & 2.91 & 3.09 & 1.9 & 3.84 & \textbf{7.58} & 2.88 & -0.01 & 8.59 & 59.45  \\
\Anybeat  & 15.58 & 15.5 & \textbf{25.8} & 14.71 & 6.36 & 15.5 & 0.0 & 8.4 & 48.07 & 7.15 & 7.1 & 8.45 & 7.1 & \textbf{9.79} & 7.22 & 0.01 & 10.23 & 83.03  \\
\CondMat  & 5.03 & 5.04 & 8.38 & \textbf{9.25} & 4.64 & 5.02 & 0.0 & 7.91 & 61.22 & 2.52 & 2.42 & 1.29 & 3.68 & \textbf{5.96} & 2.48 & 0.01 & 7.15 & 54.05  \\
\Gplus  & 1.29 & 1.29 & \textbf{21.78} & 20.7 & 20.36 & 1.31 & 0.01 & 7.77 & 42.41 & 1.97 & 1.96 & 10.48 & 11.71 & \textbf{15.03} & 2.0 & 0.01 & 10.24 & 116.28  \\
\Brightkite  & 10.49 & 10.6 & 10.44 & \textbf{11.34} & 6.31 & 10.44 & 0.03 &  \_ &  \_ & 5.93 & 5.97 & 2.82 & 5.01 & \textbf{9.91} & 5.91 & -0.0 &  - &  -  \\
\WikiTalk  & 4.82 & 4.92 & \textbf{12.07} & 7.87 & 7.71 & 4.85 & -0.04 &  \_ &  \_ & 2.62 & 2.72 & 4.61 & 5.99 & \textbf{7.01} & 2.7 & -0.13 &  - &  -  \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \end{table*}
    


==> arXiv version/tables/exp-marketing-1.tex <==
\begin{table*}[ht!]
    \caption{Results for marketing campaigns with
        $k = \lceil 0.5\%\cdot n\rceil$ seeds,
		where we initialized the innate opinions using the exponential distribution.
        We report the relative increase of each index in percent.
        }
    \label{tab:exp-marketing-1}
    \centering
      \vspace{-4mm}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c cccccccc ccccccccc}
    \toprule
    \textbf{Dataset}  & \multicolumn{8}{c}{\textbf{\sumidx}} & \multicolumn{9}{c}{\textbf{\polidx}} \\
    \cmidrule(lr){2-9} 
    \cmidrule(lr){10-18} 
      &  \MaxSum  &  \MaxLinDisCon  &  \MaxLinPol  &  \MaxLinDis  &  \MaxLinInt  &   \MaxInfluence  &  \Random  &  \FJGreedy  &  \MaxSum  &  \MaxLinDisCon  &  \MaxLinPol  &  \MaxLinDis  &  \MaxLinInt  &  \MaxInfluence  &  \Random  & \FJGreedy  & \FJUpp \\
    \midrule
\Netscience  & 6.49 & 6.59 & 2.06 & 0.25 & 0.26 & \textbf{6.65} & 0.48 & 0.25 & 8.91 & 9.17 & \textbf{38.83} & 5.38 & 2.52 & 8.98 & 0.13 & 7.29 & 86.98  \\
\WikiVote  & \textbf{7.76} & 7.75 & 0.88 & 0.8 & 0.99 & 7.74 & 0.49 & 0.2 & 2.94 & 2.81 & \textbf{14.44} & 12.13 & 0.62 & 3.05 & -0.18 & 8.58 & 55.66  \\
\Reed  & 7.05 & \textbf{7.06} & 0.71 & 0.22 & 0.83 & 7.04 & 0.6 & 0.22 & 1.4 & 1.45 & 35.55 & 31.35 & 0.24 & 1.69 & -0.04 & \textbf{37.93} & 523.59  \\
\EmailUniv  & \textbf{6.65} & 6.56 & 0.57 & 0.59 & 2.5 & 6.64 & 0.59 & 0.21 & -0.33 & -0.37 & \textbf{12.31} & 9.35 & 0.53 & 0.35 & 0.01 & 11.44 & 68.31  \\
\Hamster  & 10.27 & 10.27 & 1.69 & 1.53 & 2.61 & \textbf{10.33} & 0.7 & 0.24 & 9.87 & 9.33 & \textbf{30.42} & 22.16 & 5.26 & 9.82 & 0.06 & 20.54 & 189.96  \\
\USFCA  & 6.04 & 5.96 & 0.5 & 0.63 & 0.87 & \textbf{6.05} & 0.53 & 0.2 & 0.3 & 0.66 & \textbf{31.83} & 26.1 & 1.6 & 0.44 & -0.07 & 29.95 & 396.04  \\
\NipsEgo  & \textbf{54.35} & \textbf{54.35} & 23.57 & 2.73 & 30.95 & \textbf{54.35} & 0.45 & 0.28 & -0.77 & -0.8 & \textbf{106.59} & 20.44 & 62.12 & -0.85 & 0.14 & 6.02 & 50.36  \\
\PagesGovernment  & \textbf{8.4} & 8.34 & 2.3 & 1.39 & 1.2 & \textbf{8.4} & 0.63 & 0.23 & 11.86 & 13.21 & \textbf{29.3} & 17.34 & 4.07 & 12.18 & 0.01 & 20.98 & 265.14  \\
\HepPh  & 7.94 & 7.87 & 1.72 & 2.21 & 1.43 & \textbf{7.96} & 0.81 & 0.31 & 11.03 & 11.11 & \textbf{39.53} & 22.75 & 5.05 & 11.84 & 0.11 & 20.14 & 202.7  \\
\Anybeat  & 37.35 & 37.34 & 21.51 & 14.98 & 3.91 & \textbf{37.39} & 0.58 & 0.3 & 28.39 & 28.32 & \textbf{53.95} & 22.19 & 5.5 & 28.37 & -0.0 & 11.02 & 89.58  \\
\CondMat  & 7.92 & 7.86 & 1.77 & 1.7 & 1.06 & \textbf{7.95} & 0.74 & 0.27 & 11.38 & 12.83 & \textbf{35.5} & 17.06 & 3.91 & 12.23 & -0.03 & 15.87 & 149.43  \\
\Gplus  & 59.58 & \textbf{59.59} & 31.24 & 14.03 & 16.9 & 59.58 & 0.94 & 0.32 & 1.08 & 1.07 & \textbf{88.71} & 59.38 & 59.24 & 1.09 & -0.01 & 8.97 & 79.93  \\
\Brightkite  & 19.83 & 19.79 & 4.97 & 5.06 & 2.86 & \textbf{19.84} & 0.93 &  - & 17.2 & 17.13 & \textbf{26.8} & 16.88 & 5.54 & 17.1 & 0.06 &  - &  -  \\
\WikiTalk  & \textbf{31.54} & 31.53 & 24.23 & 0.49 & 0.49 & \textbf{31.54} & 1.2 &  - & 31.41 & 32.19 & \textbf{47.26} & 9.05 & 7.45 & 31.54 & 0.27 &  - &  -  \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \end{table*}
    


==> arXiv version/tables/exp-marketing-2.tex <==
\begin{table*}[!htb]
    \caption{Results for marketing campaigns with
        $k = \lceil 0.5\%\cdot n\rceil$ seeds,
		where we initialized the innate opinions using the exponential distribution.
        We report the relative increase of each index in percent.
	}
    \label{tab:exp-marketing-2}
    \centering
      \vspace{-4mm}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c ccccccccc ccccccccc}
    \toprule
    \textbf{Dataset}  & \multicolumn{9}{c}{\textbf{\disidx}} & \multicolumn{9}{c}{\textbf{\intidx}} \\
    \cmidrule(lr){2-10} 
    \cmidrule(lr){11-19} 
     & \MaxSum & \MaxLinDisCon & \MaxLinPol & \MaxLinDis & \MaxLinInt &  \MaxInfluence & \Random & \FJGreedy & \FJUpp & \MaxSum & \MaxLinDisCon & \MaxLinPol & \MaxLinDis & \MaxLinInt &  \MaxInfluence & \Random & \FJGreedy &\FJUpp\\
    \midrule
\Netscience  & 0.58 & 0.61 & \textbf{5.38} & 5.24 & 3.1 & 0.51 & -0.03 & 5.24 & 53.49 & -1.19 & -1.21 & -1.97 & 1.92 & \textbf{4.27} & -1.2 & -0.06 & 7.69 & 43.62  \\
\WikiVote  & 1.23 & 1.18 & 7.49 & \textbf{7.64} & 1.72 & 1.29 & -0.12 & 5.79 & 40.77 & 0.42 & 0.44 & 2.16 & 2.48 & \textbf{4.47} & 0.34 & -0.12 & 5.85 & 45.9  \\
\Reed  & 1.55 & 1.38 & 9.3 & 10.3 & 1.46 & 1.52 & 0.06 & \textbf{11.82} & 124.5 & 1.14 & 1.0 & 0.73 & 1.17 & \textbf{3.44} & 1.02 & 0.09 & 4.7 & 30.48  \\
\EmailUniv  & -0.37 & -0.49 & 4.41 & 5.89 & 2.58 & 0.1 & 0.02 & \textbf{6.15} & 39.9 & 0.07 & -0.15 & 0.78 & 2.08 & \textbf{4.66} & 0.34 & 0.05 & 4.82 & 37.14  \\
\Hamster  & 3.9 & 4.27 & 8.49 & \textbf{9.7} & 4.57 & 3.9 & -0.0 & 8.7 & 69.09 & 1.54 & 1.78 & 1.75 & 2.69 & \textbf{4.43} & 1.54 & -0.06 & 5.89 & 42.2  \\
\USFCA  & 0.01 & 0.2 & 10.18 & \textbf{11.36} & 2.01 & 0.03 & 0.0 & 11.18 & 123.72 & -0.03 & 0.01 & 1.03 & 1.63 & \textbf{3.14} & 0.05 & -0.02 & 4.26 & 29.82  \\
\NipsEgo  & -0.4 & -0.47 & 4.25 & \textbf{7.45} & 4.0 & -0.54 & 0.03 & 5.95 & 34.55 & -0.11 & -0.24 & 2.81 & \textbf{5.62} & 3.07 & -0.39 & 0.03 & 6.7 & 132.74  \\
\PagesGovernment  & 3.58 & 4.26 & \textbf{9.43} & 9.22 & 3.41 & 3.84 & 0.01 & 8.88 & 83.73 & 1.05 & 1.16 & 1.58 & 2.9 & \textbf{4.22} & 1.12 & 0.01 & 5.46 & 38.0  \\
\HepPh  & 5.54 & 6.13 & 10.95 & \textbf{12.25} & 5.33 & 5.93 & 0.02 & 10.26 & 77.54 & 2.91 & 3.09 & 1.9 & 3.84 & \textbf{7.58} & 2.88 & -0.01 & 8.59 & 59.45  \\
\Anybeat  & 15.58 & 15.5 & \textbf{25.8} & 14.71 & 6.36 & 15.5 & 0.0 & 8.4 & 48.07 & 7.15 & 7.1 & 8.45 & 7.1 & \textbf{9.79} & 7.22 & 0.01 & 10.23 & 83.03  \\
\CondMat  & 5.03 & 5.04 & 8.38 & \textbf{9.25} & 4.64 & 5.02 & 0.0 & 7.91 & 61.22 & 2.52 & 2.42 & 1.29 & 3.68 & \textbf{5.96} & 2.48 & 0.01 & 7.15 & 54.05  \\
\Gplus  & 1.29 & 1.29 & \textbf{21.78} & 20.7 & 20.36 & 1.31 & 0.01 & 7.77 & 42.41 & 1.97 & 1.96 & 10.48 & 11.71 & \textbf{15.03} & 2.0 & 0.01 & 10.24 & 116.28  \\
\Brightkite  & 10.49 & 10.6 & 10.44 & \textbf{11.34} & 6.31 & 10.44 & 0.03 &  \_ &  \_ & 5.93 & 5.97 & 2.82 & 5.01 & \textbf{9.91} & 5.91 & -0.0 &  - &  -  \\
\WikiTalk  & 4.82 & 4.92 & \textbf{12.07} & 7.87 & 7.71 & 4.85 & -0.04 &  \_ &  \_ & 2.62 & 2.72 & 4.61 & 5.99 & \textbf{7.01} & 2.7 & -0.13 &  - &  -  \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \end{table*}


==> arXiv version/tables/marketing-2.tex <==
\begin{table*}[!htb]
\caption{Results for marketing campaigns with
	$k = \lceil 0.5\%\cdot n\rceil$ seeds,
	where we initialized the innate opinions using the uniform distribution.
	We report the relative increase of each index in percent.}
\label{tab:marketing-2}
\centering
  \vspace{-4mm}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c ccccccccc ccccccccc}
\toprule
\textbf{Dataset}  & \multicolumn{9}{c}{\textbf{\disidx}} & \multicolumn{9}{c}{\textbf{\intidx}} \\
\cmidrule(lr){2-10} 
\cmidrule(lr){11-19} 
 & \MaxSum & \MaxLinDisCon & \MaxLinPol & \MaxLinDis & \MaxLinInt &  \MaxInfluence & \Random & \FJGreedy & \FJUpp & \MaxSum & \MaxLinDisCon & \MaxLinPol & \MaxLinDis & \MaxLinInt &  \MaxInfluence & \Random & \FJGreedy &\FJUpp\\
\midrule
\Netscience  & 0.81 & 0.79 & 1.21 & \textbf{1.28} & 0.44 & 0.79 & -0.12 & 1.04 &  15.84   & -0.53 & -0.54 & 0.21 & -0.13 & 0.86 & -0.53 & -0.1 & \textbf{1.1} &  16.98   \\
\WikiVote  & -1.33 & -1.32 & 1.57 & \textbf{1.77} & 0.77 & -1.28 & -0.07 & 1.12 &  15.74   & -1.47 & -1.49 & 0.35 & 0.67 & 1.0 & -1.42 & -0.08 & \textbf{1.17} &  17.84   \\
\Reed  & -0.05 & -0.09 & 2.71 & 2.59 & 0.45 & -0.08 & -0.08 & \textbf{2.74} &  44.57   & -0.39 & -0.42 & -0.0 & 0.09 & 0.69 & -0.4 & -0.08 & \textbf{0.77} &  11.49   \\
\EmailUniv  & -0.19 & -0.13 & 1.73 & \textbf{1.8} & 0.78 & -0.11 & -0.09 & 1.32 &  19.14   & -0.75 & -0.63 & 0.26 & 0.44 & \textbf{1.11} & -0.59 & -0.08 & 1.0 &  14.67   \\
\Hamster  & -0.97 & -0.93 & 1.67 & \textbf{1.87} & 0.51 & -0.81 & -0.04 & 1.45 &  22.82   & -1.14 & -1.11 & 0.12 & 0.24 & 0.67 & -1.05 & -0.07 & \textbf{0.84} &  12.85   \\
\USFCA  & -0.33 & -0.32 & 2.8 & 2.85 & 0.5 & -0.35 & -0.07 & \textbf{3.2} &  50.80   & -0.62 & -0.57 & 0.1 & 0.21 & 0.66 & -0.62 & -0.09 & \textbf{0.8} &  11.81   \\
\NipsEgo  & -5.37 & -5.35 & 0.4 & 0.55 & 0.43 & -5.35 & -0.06 & \textbf{0.71} &  10.22   & -5.33 & -5.31 & 0.38 & 0.53 & 0.83 & -5.3 & -0.06 & \textbf{1.54} &  39.06   \\
\PagesGovernment  & -0.44 & -0.44 & 2.06 & \textbf{2.26} & 0.71 & -0.56 & -0.08 & 1.83 &  29.07   & -0.81 & -0.8 & 0.18 & 0.38 & 0.75 & -0.82 & -0.08 & \textbf{0.83} &  12.67   \\
\HepPh  & -0.49 & -0.32 & 1.37 & \textbf{1.89} & 0.54 & -0.4 & -0.07 & 1.24 &  18.85   & -0.64 & -0.59 & 0.01 & 0.31 & 0.82 & -0.67 & -0.08 & \textbf{0.98} &  14.81   \\
\Anybeat  & -2.34 & -2.32 & 1.24 & \textbf{1.41} & 0.59 & -2.35 & -0.08 & 0.85 &  12.63   & -2.43 & -2.41 & 0.3 & 0.57 & 1.16 & -2.43 & -0.07 & \textbf{1.37} &  22.25   \\
\CondMat  & -0.28 & -0.21 & 1.26 & \textbf{1.77} & 0.66 & -0.27 & -0.07 & 1.15 &  17.84   & -0.68 & -0.68 & 0.03 & 0.4 & 0.81 & -0.69 & -0.07 & \textbf{0.98} &  15.40   \\
\Gplus  & -4.94 & -4.94 & \textbf{0.9} & 0.72 & 0.36 & -4.94 & -0.07 & 0.72 &  10.73   & -4.71 & -4.72 & -0.04 & 0.46 & 1.05 & -4.71 & -0.07 & \textbf{1.53} &  29.31   \\
\Brightkite  & -0.88 & -0.84 & 1.14 & \textbf{1.49} & 0.54 & -0.91 & -0.07 & - &  -   & -1.52 & -1.52 & 0.07 & 0.47 & \textbf{0.9} & -1.53 & -0.07 & - &  -   \\
\WikiTalk  & -1.43 & -1.34 & 1.66 & \textbf{1.68} & 0.61 & -1.41 & -0.09 & - &  -   & -1.94 & -1.9 & 0.38 & 0.64 & \textbf{1.06} & -1.94 & -0.09 & - &  -   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> arXiv version/tables/marketing-short.tex <==
\begin{table*}[ht!]
\caption{Results for marketing campaigns with
	$k = \lceil 0.5\%\cdot n\rceil$ seeds.
	We report the relative increase of each index in percent.}
\label{tab:marketing}
\centering
  \vspace{-4mm}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c cccccccc ccccccccc}
\toprule
\textbf{Dataset}  & \multicolumn{8}{c}{\textbf{\sumidx}} & \multicolumn{9}{c}{\textbf{\polidx}} \\
\cmidrule(lr){2-9} 
\cmidrule(lr){10-18} 
  &  \MaxSum  &  \MaxLinDisCon  &  \MaxLinPol  &  \MaxLinDis  &  \MaxLinInt  &   \MaxInfluence  &  \Random  &  \FJGreedy  &  \MaxSum  &  \MaxLinDisCon  &  \MaxLinPol  &  \MaxLinDis  &  \MaxLinInt  &  \MaxInfluence  &  \Random  & \FJGreedy  & \FJUpp \\
\midrule
\Netscience   & \textbf{2.79} & 2.75 & 0.74 & 1.01 & 0.21 & 2.78 & 0.27 & 0.11  & 3.15 & 3.18 & \textbf{7.54} & 5.89 & -0.35 & 3.17 & -0.06 & 2.36 &   10.54   \\
\WikiVote   & \textbf{4.14} & 4.12 & 0.53 & 0.64 & 0.48 & 4.11 & 0.3 & 0.11  & -0.64 & -0.61 & \textbf{3.83} & 3.2 & 0.81 & -0.58 & -0.06 & 2.92 &   12.29   \\
\Reed   & 3.2 & \textbf{3.22} & 0.28 & 0.3 & 0.3 & 3.2 & 0.27 & 0.1  & 0.14 & 0.09 & \textbf{10.13} & 8.04 & 0.15 & 0.11 & -0.13 & 9.56 &   68.48   \\
\EmailUniv   & 3.31 & \textbf{3.36} & 0.37 & 0.41 & 1.18 & 3.35 & 0.29 & 0.11  & 0.51 & 0.42 & \textbf{4.64} & 4.13 & 0.35 & 0.44 & -0.13 & 3.8 &   18.12   \\
\Hamster   & \textbf{4.09} & 4.07 & 0.76 & 0.81 & 0.45 & 4.06 & 0.27 & 0.1  & 0.39 & 0.46 & \textbf{7.59} & 5.82 & 0.43 & 0.72 & 0.01 & 5.18 &   25.70   \\
\USFCA   & 3.09 & 3.09 & 0.23 & 0.22 & 0.28 & \textbf{3.1} & 0.3 & 0.11  & -0.68 & -0.67 & \textbf{11.7} & 11.01 & 0.47 & -0.68 & -0.07 & 11.57 &   82.48   \\
\NipsEgo   & \textbf{18.75} & \textbf{18.75} & 0.47 & 0.1 & 0.1 & \textbf{18.75} & 0.15 & 0.1  & -5.3 & -5.29 & \textbf{1.71} & 0.51 & 0.12 & -5.29 & -0.09 & 0.79 &   5.34   \\
\PagesGovernment   & 3.47 & 3.47 & 0.53 & 0.5 & 0.44 & \textbf{3.48} & 0.28 & 0.1  & 0.78 & 0.79 & \textbf{7.31} & 5.49 & 0.85 & 0.51 & -0.06 & 6.96 &   36.87   \\
\HepPh   & 2.52 & \textbf{2.53} & 0.61 & 0.67 & 0.42 & 2.52 & 0.26 & 0.1  & -0.3 & 0.01 & \textbf{6.83} & 4.5 & 0.43 & -0.09 & -0.05 & 3.26 &   16.03   \\
\Anybeat   & \textbf{11.96} & \textbf{11.96} & 0.93 & 1.02 & 0.53 & \textbf{11.96} & 0.25 & 0.1  & -1.21 & -1.19 & \textbf{3.18} & 2.58 & 0.52 & -1.24 & -0.08 & 1.7 &   7.80   \\
\CondMat   & \textbf{2.79} & \textbf{2.79} & 0.59 & 0.65 & 0.48 & \textbf{2.79} & 0.25 & 0.1  & 0.35 & 0.58 & \textbf{6.9} & 4.61 & 0.44 & 0.31 & -0.07 & 3.42 &   15.69   \\
\Gplus   & \textbf{18.06} & \textbf{18.06} & 3.85 & 0.37 & 0.44 & \textbf{18.06} & 0.26 & 0.1  & -4.98 & -4.98 & \textbf{6.2} & 1.03 & 0.29 & -4.98 & -0.07 & 0.92 &   6.41   \\
\Brightkite   & 6.16 & 6.15 & 0.72 & 0.89 & 0.53 & \textbf{6.17} & 0.27 & -  & -0.17 & -0.06 & \textbf{4.27} & 2.53 & 0.47 & -0.24 & -0.07 & - &   -   \\
\WikiTalk   & 9.27 & 9.27 & 1.73 & 1.59 & 0.71 & \textbf{9.28} & 0.29 & -  & -0.82 & -0.71 & \textbf{3.37} & 2.63 & 0.62 & -0.79 & -0.09 & - &   -   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> arXiv version/tikz/epsilon/alpha1.tex <==
\pgfplotsset{compat=1.3}
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green01270}{RGB}{0,127,0}

\begin{axis}[
tick pos=both,
axis lines=left,
x grid style={darkgray176},
xmin=0.04, xmax=0.26,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0132134415500106, ymax=0.167680041387049,
ytick style={color=black},
yticklabel style = {xshift=-1ex},
legend pos= outer north east,
legend columns=1,
legend style={draw=none},
line width = 0.50 mm, 
tick style={line width=0.50mm},
ylabel={rel. increase polarization},
xlabel={$\epsilon$},
ytick scale label code/.code={$\times 10^{-2}$}
]
\addplot [black]
table {%
0.05 -0.00150354674069208
0.1 -0.00499101050741696
0.15 -0.00193440551660201
0.2 -0.00216421979118444
0.25 -4.51681235308303e-05
};
\addplot [red, dashed]
table {%
0.05 0.00183483433532726
0.1 0.00402366164020674
0.15 0.00712873072578184
0.2 0.0043399611627054
0.25 0.003464125948958
};
\addplot [blue, dotted]
table {%
0.05 0.0170610510956553
0.1 0.034780020333204
0.15 0.0508856653639139
0.2 0.0633712041020991
0.25 0.0792006936741834
};
\addplot [green01270, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
0.05 0.0325130227140441
0.1 0.063892375575521
0.15 0.0973675296817644
0.2 0.124912384461718
0.25 0.159457610344456
};
\addplot [black]
table {%
0.05 -0.000152811096278735
0.1 -0.00038046441164185
0.15 -0.000957380455787917
0.2 0.00112711389692672
0.25 0.000758960116832218
};

\addlegendentry{\MaxSum}
\addlegendentry{\MaxLinInt}
\addlegendentry{\MaxLinDis}
\addlegendentry{\MaxLinPol}
\addlegendentry{\MaxLinDisCon}


\end{axis}

\end{tikzpicture}


==> arXiv version/tikz/epsilon/alpha2.tex <==
\pgfplotsset{compat=1.3}
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green01270}{RGB}{0,127,0}

\begin{axis}[
tick pos=both,
axis lines=left,
x grid style={darkgray176},
xmin=0.04, xmax=0.26,
xtick style={color=black},
xtick = {0.05, 0.1, 0.15, 0.2, 0.25},
y grid style={darkgray176},
ymin=0.0130612900214665, ymax=0.157841545040412,
ytick style={color=black},
ytick = {0, 0.05, 0.1, 0.15},
yticklabel style = {xshift=-1ex},
legend pos= outer north east,
legend columns=1,
legend style={draw=none},
line width = 0.50 mm, 
tick style={line width=0.50mm},
ylabel={rel. increase polarization},
xlabel={$\epsilon$},
ytick scale label code/.code={$\times 10^{-2}$}
]
\addplot [black]
table {%
0.05 0.0196422107041459
0.1 0.037298196135675
0.15 0.0542923682664487
0.2 0.06261314584278
0.25 0.0786095685897592
};
\addplot [red, dashed]
table {%
0.05 0.025468871427417
0.1 0.0455394163248411
0.15 0.0645467184605504
0.2 0.078986442058507
0.25 0.092072625193864
};
\addplot [blue, dotted]
table {%
0.05 0.0317149201996606
0.1 0.0590459785490715
0.15 0.082347689311136
0.2 0.102048666437045
0.25 0.121172537738778
};
\addplot [green01270, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
0.05 0.0370309595182637
0.1 0.0712260242358546
0.15 0.102590709363027
0.2 0.130449496415652
0.25 0.151260624357733
};
\addplot [black]
table {%
0.05 0.0257338499496445
0.1 0.0471401689373272
0.15 0.0692092276787279
0.2 0.0884235948084136
0.25 0.0994291053086571
};

\addlegendentry{\MaxSum}
\addlegendentry{\MaxLinInt}
\addlegendentry{\MaxLinDis}
\addlegendentry{\MaxLinPol}
\addlegendentry{\MaxLinDisCon}

\end{axis}

\end{tikzpicture}


==> arXiv version/tikz/ttt.tex <==
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.0470588235294118,0.364705882352941,0.647058823529412}
\definecolor{color1}{rgb}{0,0.725490196078431,0.270588235294118}
\definecolor{color2}{rgb}{1,0.584313725490196,0}
\definecolor{color3}{rgb}{1,0.172549019607843,0}
\definecolor{color4}{rgb}{0.517647058823529,0.356862745098039,0.592156862745098}

\begin{axis}[
log basis y={10},
tick pos=both,
axis lines=left, xtick=\empty, ytick=\empty,
x grid style={white!69.0196078431373!black},
xmode=log,
xmin=287.974598322573, xmax=121234.106075193,
xtick style={color=black},
xtick={10,100,1000,10000,100000,1000000,10000000},
xlabel={$n$},
y grid style={white!69.0196078431373!black},
ymin=0.00270347050270336, ymax=26146.2301867163,
ymode=log,
ytick style={color=black},
ymin=0.0491058247144428, ymax=4717.94954243572,
legend style={font=\Large, draw=none},
legend pos= outer north east, 
legend columns=1,
line width = 0.50 mm, 
tick style={line width=0.50mm},
ylabel={seconds},
ytick={0.001,0.01,0.1,1,10,100,1000,10000,100000},
]
\addplot [black]
table {%
379 0.764966964721679
889 1.16822504997253
962 2.09355688095093
1133 1.3598461151123
2000 3.24952888488769
2672 15.2518429756165
2888 1.04771494865417
4158 12.8684680461884
4991 6.07284808158875
5054 12.2550020217896
7057 45.4769439697266
11204 147.640490055084
12645 38.9246850013733
14113 105.535808086395
17903 345.76726102829
21363 276.831474065781
23613 88.4117879867554
56739 476.900470018387
92117 1352.07726287842
};
\addplot [red, dashed]
table {%
379 0.300781965255737
889 4.1201479434967
962 17.492301940918
1133 6.64484000205994
2000 32.1900320053101
2672 115.749627828598
2888 21.6390209197998
4158 95.3211090564728
4991 117.369243860245
5054 199.107218027115
7057 489.44070315361
11204 1028.44246792793
12645 750.429357051849
14113 915.232490062714
17903 2702.09905195236
21363 2182.64607310295
23613 2445.63373088837
56739 652.830957174301
92117 1789.24687790871
};
\addplot [blue, dashed]
table {%
379 0.08272099494934
889 1.06456112861633
962 3.11181807518005
1133 1.66212701797485
2000 13.1593551635742
2672 67.3092830181122
2888 15.0609781742096
4158 73.0469350814819
4991 97.3521199226379
5054 199.926979064941
7057 565.310620069504
11204 991.69727897644
12645 760.318145036697
14113 880.545186042786
17903 2506.07513093948
21363 2190.7809381485
23613 2009.31821107864
56739 689.032766103745
92117 1932.56712293625
};
\addplot [green, dashed]
table {%
379 0.150960206985473
889 1.82266402244568
962 4.09466600418091
1133 4.20449185371399
2000 27.2559521198273
2672 102.760493040085
2888 18.1482269763947
4158 89.5487418174744
4991 87.510880947113
5054 184.709882974625
7057 591.682937860489
11204 980.06405210495
12645 744.870545864105
14113 876.566281080246
17903 2488.39201998711
21363 2176.75665092468
23613 2800.72553992271
56739 680.772832870483
92117 1969.11894917488
};
\addplot [red]
table {%
379 0.177518844604492
889 0.576751947402954
962 2.07290506362915
1133 1.50677299499512
2000 3.97834992408752
2672 18.1553838253021
2888 0.86129093170166
4158 19.3920450210571
4991 9.81180000305176
5054 15.1049220561981
7057 74.8052289485931
11204 215.945448160172
12645 66.7483649253845
14113 171.059938907623
17903 524.689456224442
21363 443.971834897995
23613 139.407995939255
56739 575.343125104904
92117 1477.30988001823
};
\addplot [blue]
table {%
379 0.190727949142456
889 0.567249059677124
962 2.13277697563171
1133 1.13939118385315
2000 3.90835094451904
2672 18.2101020812988
2888 0.772948026657104
4158 17.3098080158234
4991 9.41839289665222
5054 14.9316539764404
7057 69.4169249534607
11204 215.08848285675
12645 63.4836950302124
14113 167.158182144165
17903 497.33438205719
21363 422.177358865738
23613 135.526823997498
56739 573.797589063644
92117 1474.43640303612
};
\addlegendentry{\MaxSum}
\addlegendentry{\MaxLinInt}
\addlegendentry{\MaxLinDis}
\addlegendentry{\MaxLinPol}
\addlegendentry{\MaxLinDisCon}
\addlegendentry{\MaxInfluence}
\end{axis}

\end{tikzpicture}

